Collaborative Multi-Agent Reinforcement Learning for Automated Feature Transformation with Graph-Driven Path Optimization

Feature transformation methods aim to find an optimal mathematical feature-feature crossing process that generates high-value features and improves the performance of downstream machine learning tasks. Existing frameworks, though designed to mitigate manual costs, often treat feature transformations as isolated operations, ignoring dynamic dependencies between transformation steps. To address the limitations, we propose TCTO, a collaborative multi-agent reinforcement learning framework that automates feature engineering through graph-driven path optimization. The framework's core innovation lies in an evolving interaction graph that models features as nodes and transformations as edges. Through graph pruning and backtracking, it dynamically eliminates low-impact edges, reduces redundant operations, and enhances exploration stability. This graph also provides full traceability to empower TCTO to reuse high-utility subgraphs from historical transformations. To demonstrate the efficacy and adaptability of our approach, we conduct comprehensive experiments and case studies, which show superior performance across a range of datasets.

==> 7-impact.tex <==
% This paper presents work whose goal is to advance the field of Machine Learning, specifically in the area of automated feature engineering for critical domains such as healthcare prognostics and fraud detection. Our proposed framework, \model, addresses key challenges in model generalizability and labor-intensive feature engineering by introducing a collaborative multi-agent reinforcement learning approach with graph-driven path optimization. While the primary focus of this work is technical innovation, we acknowledge the broader societal implications and ethical considerations associated with advancing machine learning methodologies.

This paper presents a novel framework, aimed at advancing the field of machine learning, particularly in the automation of feature engineering.
Our approach leverages collaborative multi-agent reinforcement learning and graph-driven path optimization to address the labor-intensive nature of feature engineering. While the primary contribution is technical, we also considerate the broader societal and ethical implications of deploying such machine learning systems.

We are mindful of the ethical considerations inherent in applying machine learning to high-stakes domains. If not carefully designed and monitored, automated systems could perpetuate biases in the training data or result in unintended consequences. For example, biased models in healthcare could worsen disparities in patient care.
To mitigate these risks, we emphasize the need for transparency, traceability, and continuous evaluation of machine learning systems. The graph-driven nature of \model\ provides an inherent traceability mechanism, allowing practitioners to audit and better understand the feature transformation process.

In conclusion, our work primarily contributes to the technical advancement of machine learning, no direct ethical concerns are anticipated.
We also encourage the community to consider the ethical and societal implications of deploying such systems in real-world applications. 



==> 8-pseudo-code.tex <==
This section intends to provide the details of our methodology. 
Algorithm~\ref{alg:train} describes the optimization process of our method.
Through continuous interaction with the environment, the RGCN can effectively encode the transformation roadmap.
Cascading agents are capable of making optimal decisions based on the current state.

\begin{algorithm}[!h]
\caption{Collaborative Agents Optimization Phase}
\label{alg:train}
\textbf{Input}: dataset $\mathcal{D}[\mathcal{F},Y]$\\
\textbf{Initialization}: downstream ML task $\mathcal{M}$, evaluation metric $\mathcal{V}$, complexity metric $\mathcal{U}$, head cluster agent $\pi_{h}$, operation agent $\pi_{o}$, operand cluster agent $\pi_{t}$, cluster state representation $Rep(\cdot)$, reward $\mathcal{R}$\\
\textbf{Parameter}: training episode T, training step N, prune strategy node number p \\
\textbf{Output}: head cluster agent $\pi_{h}$, operation agent $\pi_{o}$, operand cluster agent $\pi_{t}$, RGCN encoder $Rep(\cdot)$
\begin{algorithmic}[1] %[1] enables line numbers
\FOR{$i=0$ to $T$}
    \STATE $\mathcal{G} \gets \mathcal{D}$ {\hfill\color{gray} \# 1. Initialize roadmap based on dataset} 
    \FOR{$j=0$ to $N$}
        \STATE $\mathcal{C} \gets $ clustering roadmap $\mathcal{G}$ 
        \STATE $c_h \gets \pi_{h}(Rep(\mathcal{G}),Rep(C))$ {\hfill\color{gray}\# 2. Head agent decision} 
        \STATE $o \gets \pi_{o}(Rep(\mathcal{G}),Rep(C),Rep(c_h))$ {\hfill\color{gray} \# 3. Operation agent decision} 
        \IF{$o$ is a unary operation}
            \STATE $\mathcal{D} \gets (\mathcal{D} \cup (o \rightarrow c_h))$ {\hfill\color{gray}\# 4. Generate new features and update dataset} \ \
        \ELSE 
            \STATE 
            $c_t \gets \pi_{t}(Rep(\mathcal{G}),Rep(C),Rep(c_h),Rep(o))$ {\hfill\color{gray}\# 5. Operand agent decision}
            \STATE 
            $\mathcal{D} \gets (\mathcal{D} \cup (c_h \rightarrow o  \rightarrow c_t))$ 
            {\hfill\color{gray}\# 6. Generate new features and update dataset} \ \
        \ENDIF
        \STATE $\mathcal{G}$ \ \ \  UPDATES
        \STATE $\mathcal{R} \gets \mathcal{R}_p + \mathcal{R}_c$
        {\hfill\color{gray}\# 7. Calculate combining reward}
        \STATE Optimize $\pi_{h}$, $\pi_{o}$, $\pi_{t}$ and encoder $Rep$ based on $\mathcal{R}$
        \IF{node number of $\mathcal{G} >$ p}
            \STATE $\mathcal{G} \gets Prune\ \mathcal{G}$
            % \IF{$i < w$}
            %     \STATE $\mathcal{G} \gets P_{n}(\mathcal{G})$ {\hfill\color{gray}\# 9. Node-wise prune strategy}
            % \ELSE
            %     \STATE $\mathcal{G} \gets P_{s}(\mathcal{G})$ {\hfill\color{gray} \# 10. Step-wise prune strategy}
            % \ENDIF
        \ENDIF
    \ENDFOR
\ENDFOR
\STATE \textbf{return} $\pi_{h}$, $\pi_{o}$, $\pi_{t}$, $Rep$
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:test} describes the application process of \model{}.
The optimized reinforcement learning agents can make decisions based on the current roadmap, resulting in a dataset with better performance on downstream tasks.

\begin{algorithm}[!h]
\caption{Collaborative Agents Application Phase}
\label{alg:test}
\textbf{Input}: dataset $\mathcal{D}[\mathcal{F},Y]$, head cluster agent $\pi_{h}$, operation agent $\pi_{o}$, operand cluster agent $\pi_{t}$, cluster state representation $Rep(\cdot)$\\
\textbf{Initialization}: downstream ML task $\mathcal{M}$, evaluation metric $\mathcal{V}$, complexity metric $\mathcal{U}$\\
\textbf{Parameter}: testing episode T, testing step N, prune strategy node number p\\
\textbf{Output}: optimal dataset $\mathcal{D}^{'}$
\begin{algorithmic}[1] %[1] enables line numbers
\FOR{$i=0$ to $T$}
    \STATE $\mathcal{G} \gets \mathcal{D}$ 
    {\hfill\color{gray} \# 1. Initialize roadmap based on dataset}
    \STATE Let best performance $m=0$, current best dataset $D^{'}=D$.
    \FOR{$j=0$ to $N$}
        \STATE $\mathcal{C} \gets $ clustering roadmap $\mathcal{G}$ 
        \STATE $c_h \gets \pi_{h}(Rep(\mathcal{G}),Rep(C))$  {\hfill\color{gray} \# 2. Head agent decision}
        \STATE $o \gets \pi_{o}(Rep(\mathcal{G}),Rep(C),Rep(c_h))$ {\hfill\color{gray} \# 3. Operation agent decision} 
        \IF{$o$ is a unary operation}
            \STATE $\mathcal{D} \gets (\mathcal{D} \cup (o \rightarrow c_h))$ 
            {\hfill\color{gray} \# 4. Generate new features } 
        \ELSE
            \STATE  
            $c_t \gets \pi_{o}(Rep(\mathcal{G}),Rep(C),Rep(c_h),Rep(o))
            ${\hfill\color{gray}  \# 5. Tail agent decision}
            \STATE  
            $\mathcal{D} \gets (\mathcal{D} \cup (c_h \rightarrow o  \rightarrow c_t))
            ${\hfill\color{gray}  \# 6. Generate new features} \ \ 
        \ENDIF
        \STATE $\mathcal{G}$ \ \ \  UPDATES
        \IF{$\mathcal{V}(\mathcal{M}(\mathcal{D})) > m$}
            \STATE $m \gets \mathcal{V}(\mathcal{M}(\mathcal{D}))$
            \STATE $D^{'} \gets D$ 
            {\hfill\color{gray} \# 7. Update optimal dataset} \ \ 
        \ENDIF
        \IF{node number of $\mathcal{G} >$ p}
            \STATE $\mathcal{G} \gets Prune\ \mathcal{G}$
        \ENDIF
    \ENDFOR
\ENDFOR
\STATE \textbf{return} $\mathcal{D}^{'}$
\end{algorithmic}
\end{algorithm}
